Ready for Rain? A View from SPEC Research on the Future of Cloud Metrics

In the past decade, cloud computing has emerged from a pursuit for a service-driven information and communication technology (ICT), into a signifcant fraction of the ICT market. Responding to the growth of the market, many alternative cloud services and their underlying systems are currently vying for the attention of cloud users and providers. Thus, benchmarking them is needed, to enable cloud users to make an informed choice, and to enable system DevOps to tune, design, and evaluate their systems. This requires focusing on old and new system properties, possibly leading to the re-design of classic benchmarking metrics, such as expressing performance as throughput and latency (response time), and the design of new, cloud-specififc metrics. Addressing this requirement, in this work we focus on four system properties: (i) elasticity of the cloud service, to accommodate large variations in the amount of service requested, (ii) performance isolation between the tenants of shared cloud systems, (iii) availability of cloud services and systems, and the (iv) operational risk of running a production system in a cloud environment.Focusing on key metrics, for each of these properties we review the state-of-the-art, then select or propose new metrics together with measurement approaches. We see the presented metrics as a foundation towards upcoming, industry-standard, cloud benchmarks. Keywords: Cloud Computing; Metrics; Measurement; Benchmarking; Elasticity; Isolation; Performance; Service Level Objective; Availability; Operational Risk.

==> researchChallenges.tex <==
\chapter{Research challenges}

\begin{itemize}
	\item Definition of cloud-specific metrics
	\item $\rightarrow$ elasticity
	\item $\rightarrow$ isolation
	\item $\rightarrow$ \ldots
	\item Time as new benchmark dimension 
	\item $\rightarrow$ unique nature of elasticity benchmarking
	\item $\rightarrow$ $\rightarrow$ not only high low is important, but also low and mid and the transitions between them.
	\item $\rightarrow$ $\rightarrow$ the speed of the transitions need to vary too
	\item $\rightarrow$ when the benchmark is done - differences in benchmarking in peak or low times -> important for clouds
	\item $\rightarrow$ need of not only continuous change of workload from low to peak, but also intense, sudden changes
	\item $\rightarrow$ $\rightarrow$ examples from real world why sudden changes would occur (very popular game, protest against services, changes in prices - promotions etc)
	\item Problem
	\item $\rightarrow$ scalability of the benchmark - The SUT may grow and handle virtually unlimited loads 
	\item $\rightarrow$ stability and \textbf{repeatability} of benchmark (results)
	\item $\rightarrow$ for some cloud benchmark types (like SaaS, but maybe also PaaS and IaaS), the box is completely black. More black then in all other traditional benchmarks. For example, we have no control what is running on background, or with how many tenants we share the machine.
	\item SaaS benchmarking
	\item $\rightarrow$ Identification of comparability characteristics in SaaS benchmarks
	\item $\rightarrow$ Benchmarking software with similar characteristics
	\item $\rightarrow$ $\rightarrow$ In aspect of what they offer to the user (functionality, e.g. mail)
	\item $\rightarrow$ $\rightarrow$ In aspect of how they are made
	\item $\rightarrow$ Long-term availability of the software (Facebook games can be popular once and not popular later)
	\item Future Extensions
	\item $\rightarrow$ state that not everything is here
	\item $\rightarrow$ more work can be done...
\end{itemize}
